Estimating brain age based on a healthy population with deep learning and structural MRI

Numerous studies have established that estimated brain age, as derived from statistical models trained on healthy populations, constitutes a valuable biomarker that is predictive of cognitive decline and various neurological diseases. In this work, we curate a large-scale heterogeneous dataset (N = 10,158, age range 18 - 97) of structural brain MRIs in a healthy population from multiple publicly-available sources, upon which we train a deep learning model for brain age estimation. The availability of the large-scale dataset enables a more uniform age distribution across adult life-span for effective age estimation with no bias toward certain age groups. We demonstrate that the age estimation accuracy, evaluated with mean absolute error (MAE) and correlation coefficient (r), outperforms previously reported methods in both a hold-out test set reflective of the custom population (MAE = 4.06 years, r = 0.970) and an independent life-span evaluation dataset (MAE = 4.21 years, r = 0.960) on which a previous study has evaluated. We further demonstrate the utility of the estimated age in life-span aging analysis of cognitive functions. Furthermore, we conduct extensive ablation tests and employ feature-attribution techniques to analyze which regions contribute the most predictive value, demonstrating the prominence of the frontal lobe as well as pattern shift across life-span. In summary, we achieve superior age estimation performance confirming the efficacy of deep learning and the added utility of training with data both in larger number and more uniformly distributed than in previous studies. We demonstrate the regional contribution to our brain age predictions through multiple routes and confirm the association of divergence between estimated and chronological brain age with neuropsychological measures.

==> sections/abstract_long.tex <==

Numerous studies have established that estimated brain age,
as derived from statistical models trained on healthy populations,
constitutes a valuable biomarker 
that is predictive of cognitive decline 
and various neurological diseases.
In this work, we curate a large-scale heterogeneous dataset (N = 10,158, age range 18 - 97)
of structural brain MRIs in a healthy population from multiple publicly-available sources,
upon which we train a deep learning model for brain age estimation.
The availability of the large-scale dataset 
enables a more uniform age distribution across adult life-span 
for effective age estimation
with no bias toward certain age groups.
We demonstrate that the age estimation accuracy, evaluated with mean absolute error (MAE) and correlation coefficient (\emph{r}),
outperforms previously reported methods in both
a hold-out test set reflective of the custom population (MAE = 4.06 years, \emph{r} = 0.970) and
an independent life-span evaluation dataset (MAE = 4.21 years, \emph{r} = 0.960) on which a previous study has evaluated.
We further demonstrate the utility of the estimated age 
in life-span aging analysis of cognitive functions.
Our analysis demonstrates that 
divergence of the estimated age from the chronological age 
is associated with neuropsychological measures 
after controlling for the chronological age.
Furthermore, we conduct extensive ablation tests 
and employ feature-attribution techniques 
to analyze which regions contribute the most predictive value,
demonstrating the prominence of the frontal lobe 
as well as pattern shift across life-span.

In summary, 
we achieve superior age estimation performance 
confirming the efficacy of deep learning and
the added utility of training with data both in larger number 
and more uniformly distributed than in previous studies.
We demonstrate the regional contribution to our brain age predictions 
through multiple routes and confirm the association 
of deviations between estimated and chronological brain age 
with neuropsychological measures.
Further study may expand the value of age estimation 
for other correlates of brain insult or function 
across a variety of structural scans, 
as well as provide an additional metric useful in studying aging itself.


